SoK: Scalability Techniques for BFT Consensus

With the advancement of blockchain systems, many recent research works have proposed distributed ledger technology~(DLT) that employs Byzantine fault-tolerant~(BFT) consensus protocols to decide which block to append next to the ledger. Notably, BFT consensus can offer high performance, energy efficiency, and provable correctness properties, and it is thus considered a promising building block for creating highly resilient and performant blockchain infrastructures. Yet, a major ongoing challenge is to make BFT consensus applicable to large-scale environments. A large body of recent work addresses this challenge by developing novel ideas to improve the scalability of BFT consensus, thus opening the path for a new generation of BFT protocols tailored to the needs of blockchain. In this survey, we create a systematization of knowledge about the novel scalability-enhancing techniques that state-of-the-art BFT consensus protocols use. For our comparison, we closely analyze the efforts, assumptions, and trade-offs these protocols make.

==> sections/table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%\begin{sidewaystable*}[p]
\begin{table*}[t]
\centering
\caption{Comparison of scalable \ac{BFT} protocols regarding their assumptions, goals, and scaling techniques.}
\label{tab:protocols}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|
>{\columncolor[HTML]{C9FEFC}}c 
>{\columncolor[HTML]{C9FEFC}}c 
>{\columncolor[HTML]{C9FEFC}}c |
>{\columncolor[HTML]{E0FFE0}}c 
>{\columncolor[HTML]{E0FFE0}}c |
>{\columncolor[HTML]{FFFFC7}}c 
>{\columncolor[HTML]{FFFFC7}}c 
>{\columncolor[HTML]{FFFFC7}}c 
%>{\columncolor[HTML]{FFFFC7}}c 
>{\columncolor[HTML]{FFFFC7}}c 
>{\columncolor[HTML]{FFFFC7}}c 
>{\columncolor[HTML]{FFFFC7}}c |}
\hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} } &
  \multicolumn{3}{c|}{\cellcolor[HTML]{\colorassumption}{\color[HTML]{000000} \textbf{Assumptions}}} &
  \multicolumn{2}{c|}{\cellcolor[HTML]{\colorguarantees}{\color[HTML]{000000} \textbf{Guarantees}}} &
  \multicolumn{6}{c|}{\cellcolor[HTML]{\colorscaling}{\color[HTML]{000000} \textbf{Scaling Techniques}}} \\ \cline{2-13} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}BFT\\ Protocol\end{tabular}}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{\colorassumption}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Network (for\\ safety+liveness)\end{tabular} }}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{\colorassumption}{\color[HTML]{000000} \textbf{Fault}}} &
  {\color[HTML]{000000} \textbf{Members}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{\colorguarantees}{\color[HTML]{000000} \textbf{Safety}}} &
  {\color[HTML]{000000} \textbf{Liveness}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{\colorscaling}{\color[HTML]{000000} \textbf{Leader}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{\colorscaling}{\color[HTML]{000000} \textbf{Crypto}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{\colorscaling}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Message\\ Exchange\end{tabular}}}} &
  %\multicolumn{1}{c|}{\cellcolor[HTML]{\colorscaling}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Pipelining\\ Strategy\end{tabular}}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{\colorscaling}{\color[HTML]{000000} \textbf{Consensus}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{\colorscaling}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Parallel\\ -ization\end{tabular}}}} &
  \textbf{Other} \\ \hline


% Title &
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline


% \iffalse
% %%% THESE are surveys and I guess they should not be in this table...
% A Survey on Consortium Blockchain Consensus Mechanisms &
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline

% The Quest for Scalable Blockchain Fabric: Proof-of-Work vs. BFT Replication &
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline

% Scaling Byzantine Consensus: A Broad Analysis &
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline
% `
% Scaling Blockchains: A Comprehensive Survey &
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline
% \fi 


% Beginn: CB checking
% Enhancing Bitcoin Security and Performance with Strong Consistency via Collective Signing &
ByzCoin \cite{kogias2016enhancing} 
%\hr{ich wäre ja für diese Kurzform Kurzname + Referenz }\av{So hatten wir das glaube ich auch abgemacht, das hat sich aber leider nicht automatisieren lassen} 
&
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfpowbound} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\doublecell{\leadersingle}{\leaderpowelected}} & % leader
\cell{\colorscaling}{\cryptomultisignature} & % crypto
\cell{\colorscaling}{\exchangetree} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%Scalable and leaderless Byzantine consensus in cloud computing environments &
Lim et al.~\cite{lim2014scalable} &
\cell{\colorassumption}{\networkasync} & % network assumptions. cb: no explicits assumptions in paper found -> async? Algorithm descriptions also do not use timers etc.
\cell{\colorassumption}{\maxfhalf} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadernone} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{\exchangegossip} & % message exchange
\cell{\colorscaling}{\consensusrandomizedsampling} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline
 
%The design, architecture and performance of the Tendermint Blockchain Network &
Tendermint \cite{buchman2016tendermint} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\doublecell{\leadersingle}{\leaderrotating}} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{\exchangegossip} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%RepChain: A Reputation-Based Secure, Fast, and High Incentive Blockchain System via Sharding &
RepChain \cite{huang2021repchain} &
\cell{\colorassumption}{\networksync} & %{\doublecell{\networkpartialsync}{\networksync}} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptomultisignature} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

% cb: Should this really be included in survey? Discuss
%Ostraka: Secure Blockchain Scaling by Node Sharding &
Ostraka \cite{manuskin2020ostraka} &
\cell{\colorassumption}{\todo{\conf}} & % network assumptions
\cell{\colorassumption}{\maxfhalf} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{-/\todo{\conf}} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic/\todo{\conf}} & % liveness guarantees
\cell{\colorscaling}{\todo{\conf}} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline


%Mitosis: Practically Scaling Permissioned Blockchains &
Mitosis \cite{marson2021mitosis} &
\cell{\colorassumption}{\networkpartialsync/\todo{\conf}} & % network assumptions
\cell{\colorassumption}{\maxfparameterizable} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{-/\todo{\conf}} & % safety guarantees
\cell{\colorguarantees}{-/\todo{\conf}} & % liveness guarantees
\cell{\colorscaling}{\todo{\conf}} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%Kauri: Scalable BFT Consensus with Pipelined Tree-Based Dissemination and Aggregation &
Kauri \cite{neiheiser2021kauri} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptomultisignature} & % crypto
\cell{\colorscaling}{\exchangetree} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\doublecell{configurable pipe-} {lining stretch}}  % other
 \\ \hline

%HotStuff: BFT Consensus with Linearity and Responsiveness &
HotStuff \cite{hotstuff19} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\doublecell{\leadersingle}{\leaderrotating}} & % leader
\cell{\colorscaling}{\cryptothreshold} & % crypto
\cell{\colorscaling}{\exchangestar} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\doublecell{one pipeline stage}{per protocol stage}}  % other
 \\ \hline




%A Scalable Multi-Layer PBFT Consensus for Blockchain &
X-Layer PBFT \cite{li2020scalable} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfparameterizable} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{\exchangetree} & % message exchange
\cell{\colorscaling}{\consensushierarchical} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

% \iffalse
% A Comparison of Message Exchange Patterns in BFT Protocols: (Experience Report) &
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline
% \fi



%A Blockchain Consensus Protocol With Horizontal Scalability &
CHECO \cite{cong2018blockchain} &
\cell{\colorassumption}{\networkasync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadermulti} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline


%Beh-Raft-Chain: A Behavior-Based Fast Blockchain Protocol for Complex Networks &
Beh-Raft-Chain \cite{wang2021behraftchain} &
\cell{\colorassumption}{\networksync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptovrf} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensushierarchical} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%An Optimized Byzantine Fault Tolerance Algorithm for Consortium Blockchain 
SHBFT \cite{li2021optimized}&
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfunk} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{?} & % safety guarantees
\cell{\colorguarantees}{?} & % liveness guarantees
\cell{\colorscaling}{\doublecell{\leadersingle}{\leadermulti}} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensushierarchical} & % consensus
\cell{\colorscaling}{\parallelizationhierachicalconsensus} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline


% The Hermes BFT for Blockchains &
Hermes BFT \cite{jalalzai2021hermes} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensuscommittee} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\doublecell{chain-based}{pipelining}}  % other
 \\ \hline


%continue here

% %The Meshwork Ledger, its Consensus and Reward Mechanisms &
% Meshwork Ledger \cite{raikwar2021meshwork} \todo{wasn't this marked as a conflict and discarded?} &
% \cell{\colorassumption}{\networkpartialsync} & % network assumptions
% \cell{\colorassumption}{\maxfthird} & % fault tolerance
% \cell{\colorassumption}{\membershipdynamic} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{\leadersingle} & % leader
% \cell{\colorscaling}{\cryptomultisignature} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline

% \iffalse
% SoK: Sharding on Blockchain &
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline
% \fi

%SharPer: Sharding Permissioned Blockchains Over Network Clusters &
SharPer \cite{amiri2021sharper} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

FastBFT \cite{liu2018scalable} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfhalf} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptosecretsharing} & % crypto
\cell{\colorscaling}{\exchangetree} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{HW/TEE}  % other
 \\ \hline

%continue here
%ResilientDB: global scale resilient blockchain fabric &
ResilientDB \cite{gupta2020resilientdb} &
\cell{\colorassumption}{\networksync} & % network assumptions
\cell{\colorassumption}{\maxfresdb} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadermulti} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationclustering} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline
 
BFT-Store~\cite{qi2020reliable} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfparameterizable} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\doublecell{\leadersingle}{\leaderrotating}} & % leader
\cell{\colorscaling}{\cryptoerasurecoding} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\doublecell{storage}{scalability}}  % other
 \\ \hline
 
 % END CB checking

%Red Belly: A Secure, Fair and Scalable Open Blockchain &
Red Belly~\cite{crain2021red} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadernone} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%RCC: Resilient Concurrent Consensus for High-Throughput Secure Transaction Processing &
RCC \cite{rcc2021gupta} &
\cell{\colorassumption}{\networkpartialsync/\todo{\conf}} & % network assumptions
\cell{\colorassumption}{\maxfthird/\todo{\conf}} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadermulti} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\doublecell{Concurrent}{processing}} & % parallelization
\cell{\colorscaling}{(PBFT Variant)}  % other
 \\ \hline

%RapidChain: Scaling Blockchain via Full Sharding &
RapidChain~\cite{zamani2018rapidchain} &
\cell{\colorassumption}{\networksync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\doublecell{\leadersingle}{\leaderrandomselection}} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{\exchangegossip} & % message exchange
\cell{\colorscaling}{\consensuscommittee} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{\doublecell{intrashard}{pipelining}}  % other
 \\ \hline

%Pyramid: A Layered Sharding Blockchain System &
Pyramid~\cite{hong2021pyramid} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadermulti} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%Proteus: A Scalable BFT Consensus Protocol for Blockchains &
Proteus~\cite{jalalzai2019proteus} &
\cell{\colorassumption}{\networkasync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{\exchangestar} & % message exchange
\cell{\colorscaling}{\consensuscommittee} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%Proof-of-QoS: QoS based blockchain consensus protocol &
Proof-of-QoS~\cite{yu2019proofofqos} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird~per committee} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptovrf} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensuscommittee} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%Proof-of-Execution: Reaching Consensus through Fault-Tolerant Speculation &
Proof-of-Execution~\cite{gupta2021poe} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptothreshold} & % crypto
\cell{\colorscaling}{\exchangestar} & % message exchange
\cell{\colorscaling}{\consensusspeculativeexecution} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\doublecell{Out-of-order}{processing}}  % other
 \\ \hline

Musch~\cite{jalalzai2018window} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptomultisignature} & % crypto
\cell{\colorscaling}{\exchangestar} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

AHL~\cite{dang2019towards} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptomultisignature} & % crypto
\cell{\colorscaling}{\exchangestar} & % message exchange
\cell{\colorscaling}{\consensuscommittee} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{HW/TEE}  % other
 \\ \hline

%Dumbo: Faster Asynchronous BFT Protocols &
Dumbo~\cite{guo2020dumbo} &
\cell{\colorassumption}{\networkasync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadermulti} & % leader
\cell{\colorscaling}{\doublecell{\cryptoerasurecoding}{\cryptothresholdencryption}} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensuscommittee} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%DP-Hybrid: A Two-Layer Consensus Protocol for High Scalability in Permissioned Blockchain &
DP-Hybrid~\cite{zheng2020dphybrid} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfparameterizable} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\doublecell{\leadernone}{\leadersingle}} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensushierarchical} & % consensus
\cell{\colorscaling}{\parallelizationhierachicalconsensus} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%DLattice: A Permission-Less Blockchain Based on DPoS-BA-DAG Consensus for Data Tokenization &
DLattice \cite{zhou2019dlattice} &
\cell{\colorassumption}{\networksync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadernone} & % leader
\cell{\colorscaling}{\cryptovrf} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensuscommittee} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%DBFT: Efficient Leaderless Byzantine Consensus and its Application to Blockchains &
DBFT~\cite{crain2018dbft} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadernone} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%Cumulus: A Secure BFT-based Sidechain for Off-chain Scaling &
Cumulus~\cite{gai2021cumulus} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\doublecell{\cryptothreshold}{\cryptovrf}} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%Chainspace: A Sharded Smart Contracts Platform &
Chainspace~\cite{al-bassam2018chainspace} &
\cell{\colorassumption}{\networkasync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%CAPER: a cross-application permissioned blockchain &
CAPER~\cite{amiri2019caper} &
\cell{\colorassumption}{\networkasync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensushierarchical} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%BlockTree: a nonlinear structured, scalable and distributed ledger scheme for processing digital transactions &
BlockTree~\cite{blocktree2021vishwakarma} &
\cell{\colorassumption}{\networkasync} & % network assumptions
\cell{\colorassumption}{\maxfhalf} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%Dispel: Byzantine SMR with Distributed Pipelining &
Dispel~\cite{voron2019dispel} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadernone} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\doublecell{\textit{distributed}}{pipeline}}  % other
 \\ \hline
 
 % \todo{start signe}
%BigBFT: A Multileader Byzantine Fault Tolerance Protocol for High Throughput &
BigBFT \cite{alqahtani2021bigbft} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadermulti} & % leader
\cell{\colorscaling}{\cryptomultisignature} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\doublecell{pipelining blocks}{across rounds}}  % other
 \\ \hline

% Gosig: Scalable Byzantine Consensus on Adversarial Wide Area Network for Blockchains &
Gosig \cite{li2020gosig} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leaderrandomselection} & % leader
\cell{\colorscaling}{\cryptomultisignature} & % crypto
\cell{\colorscaling}{\exchangegossip} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\doublecell{pipelines gossiplayer}{\textit{and} BFT protocol}}  % other
 \\ \hline

%RingBFT: Resilient Consensus over Sharded Ring Topology &
RingBFT \cite{rahnama2021ringbft} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{\exchangering} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%DispersedLedger: High-Throughput Byzantine Consensus on Variable Bandwidth Networks &
DispersedLedger \cite{yang2022dispersed} &
\cell{\colorassumption}{\networkasync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadernone} & % leader
\cell{\colorscaling}{\cryptoerasurecoding} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%Saguaro: Efficient Processing of Transactions in Wide Area Networks using a Hierarchical Permissioned Blockchain &
Saguaro \cite{amiri2021saguaro} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptothreshold} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensushierarchical} & % consensus
\cell{\colorscaling}{\parallelizationhierachicalconsensus} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

% Evaluating the Red Belly Blockchain \sr{duplicate with red belly \cite{crain2021red}?} &
% \cell{\colorassumption}{\networkpartialsync} & % network assumptions
% \cell{\colorassumption}{\maxfthird} & % fault tolerance
% \cell{\colorassumption}{\membershipdynamic} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{\leadernone} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{\parallelizationsharding} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline

%Qanaat: A Scalable Multi-Enterprise Permissioned Blockchain System with Confidentiality Guarantees &
Qanaat \cite{amiri2021qanaat} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptosecretsharing} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

% Building Blocks of Sharding Blockchain Systems: Concepts, Approaches, and Open Problems \sr{related work / survey} &
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline

% %Betting on Blockchain Consensus with Fantomette&
% Fantomette \cite{azouvi2018fantomette} \todo{conflict} &
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline

Narwhal-HotStuff \cite{danezis2022narwhal} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leaderrotating} & % leader
\cell{\colorscaling}{\cryptothreshold} & % crypto
\cell{\colorscaling}{\exchangestar} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\pipelininghotstuff}  % other
 \\ \hline

Tusk \cite{danezis2022narwhal} &
\cell{\colorassumption}{\networkasync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leaderrotating} & % leader
\cell{\colorscaling}{\cryptothreshold} & % crypto
\cell{\colorscaling}{\exchangestar} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\pipelininghotstuff}  % other
 \\ \hline

Avalanche \cite{rocket2020avalanche} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfparameterizable} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadernone} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{\exchangegossip} & % message exchange
\cell{\colorscaling}{\consensusrandomizedsampling} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

% The quest for scaling BFT Consensus through Tree-Based Vote Aggregation \sr{duplicate with Kauri} &
% \cell{\colorassumption}{\networkpartialsync} & % network assumptions
% \cell{\colorassumption}{\maxfthird} & % fault tolerance
% \cell{\colorassumption}{\membershipstatic} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{\leadersingle} & % leader
% \cell{\colorscaling}{\cryptobls} & % crypto
% \cell{\colorscaling}{\exchangetree} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline

% Concurrent Practical Byzantine Fault Tolerance for Integration of Blockchain and Supply Chain 
C-PBFT \cite{xu2021concurrent} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensushierarchical} & % consensus
\cell{\colorscaling}{\parallelizationhierachicalconsensus} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

% Byzantine Agreement with Less Communication: Recent Advances \sr{related work / survey}&
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline

%DRBFT: Delegated randomization Byzantine fault tolerance consensus protocol for blockchains &
DRBFT \cite{zhan2021drbft} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\doublecell{\consensuscommittee}{\consensusrandomizedsampling}} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

%SBFT: a Scalable Decentralized Trust Infrastructure for Blockchains &
SBFT \cite{gueta2019sbft} &
\cell{\colorassumption}{\networksync} & % network assumptions
\cell{\colorassumption}{\maxfSBFT} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptothreshold} & % crypto
\cell{\colorscaling}{\exchangestar} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\doublecell{learning heuristic} {for dynamic batching}}  % other
 \\ \hline

% Cerberus: Minimalistic Multi-shard Byzantine-resilient Transaction Processing &
Cerberus \cite{hellings2020cerberus} &
\cell{\colorassumption}{\networkasync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

% GearBox: An Efficient UC Sharded Ledger Leveraging the Safety-Liveness Dichotomy &
GearBox \cite{david2021gearbox} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensuscommittee} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

% ByShard: Sharding in a Byzantine Environment &
ByShard \cite{hellings2021byshard} &
\cell{\colorassumption}{\conf} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\conf} & % node membership
\cell{\colorguarantees}{\conf} & % safety guarantees
\cell{\colorguarantees}{\conf} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{-} & % crypto
\cell{\colorscaling}{-} & % message exchange
\cell{\colorscaling}{\consensushierarchical} & % consensus
\cell{\colorscaling}{\parallelizationsharding} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

ICC0 / ICC1 \cite{camenisch2022internet} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\doublecell{\leadersingle}{\leaderrotating}} & % leader
\cell{\colorscaling}{\cryptothreshold} & % crypto
\cell{\colorscaling}{\exchangegossip} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

ICC2 \cite{camenisch2022internet} &
\cell{\colorassumption}{\networkpartialsync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetydeterministic} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\doublecell{\leadersingle}{\leaderrotating}} & % leader
\cell{\colorscaling}{\doublecell{\cryptothreshold}{\cryptoerasurecoding}} & % crypto
\cell{\colorscaling}{\exchangegossip} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-}  % other
 \\ \hline

Jolteon \cite{gelashvili2021jolteon} &
\cell{\colorassumption}{{\networkpartialsync}} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{{\safetydeterministic}} & % safety guarantees
\cell{\colorguarantees}{\safetydeterministic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptothreshold} & % crypto
\cell{\colorscaling}{\exchangestar} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\pipelininghotstuff}  % other
 \\ \hline

Ditto \cite{gelashvili2021jolteon} &
\cell{\colorassumption}{{\networkasync}} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipstatic} & % node membership
\cell{\colorguarantees}{{\safetyprobabilistic}} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leadersingle} & % leader
\cell{\colorscaling}{\cryptothreshold} & % crypto
\cell{\colorscaling}{\exchangestar} & % message exchange
\cell{\colorscaling}{-} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{\pipelininghotstuff}  % other
 \\ \hline

% \iffalse
% Recent advances in consensus protocols for blockchain: a survey &
% \cell{\colorassumption}{-} & % network assumptions
% \cell{\colorassumption}{-} & % fault tolerance
% \cell{\colorassumption}{-} & % node membership
% \cell{\colorguarantees}{-} & % safety guarantees
% \cell{\colorguarantees}{-} & % liveness guarantees
% \cell{\colorscaling}{-} & % leader
% \cell{\colorscaling}{-} & % crypto
% \cell{\colorscaling}{-} & % message exchange
% \cell{\colorscaling}{-} & % consensus
% \cell{\colorscaling}{-} & % parallelization
% \cell{\colorscaling}{-}  % other
%  \\ \hline
% \fi 

% Algorand: Scaling Byzantine Agreements for Cryptocurrencies &
Algorand \cite{gilad2017algorand} &
\cell{\colorassumption}{\networksync} & % network assumptions
\cell{\colorassumption}{\maxfthird} & % fault tolerance
\cell{\colorassumption}{\membershipdynamic} & % node membership
\cell{\colorguarantees}{\safetyprobabilistic} & % safety guarantees
\cell{\colorguarantees}{\safetyprobabilistic} & % liveness guarantees
\cell{\colorscaling}{\leaderrandomselection} & % leader
\cell{\colorscaling}{\cryptovrf} & % crypto
\cell{\colorscaling}{\exchangegossip} & % message exchange
\cell{\colorscaling}{\consensuscommittee} & % consensus
\cell{\colorscaling}{-} & % parallelization
\cell{\colorscaling}{-} %other
\\ \hline

\end{tabular}%
}
\end{table*}
%\end{sidewaystable*}
